Evaluating Software Development Agents: Patch Patterns, Code Quality, and Issue Complexity in Real-World GitHub Scenarios

In recent years, AI-based software engineering has progressed from pre-trained models to advanced agentic workflows, with Software Development Agents representing the next major leap. These agents, capable of reasoning, planning, and interacting with external environments, offer promising solutions to complex software engineering tasks. However, while much research has evaluated code generated by large language models (LLMs), comprehensive studies on agent-generated patches, particularly in real-world settings, are lacking. This study addresses that gap by evaluating 4,892 patches from 10 top-ranked agents on 500 real-world GitHub issues from SWE-Bench Verified, focusing on their impact on code quality. Our analysis shows no single agent dominated, with 170 issues unresolved, indicating room for improvement. Even for patches that passed unit tests and resolved issues, agents made different file and function modifications compared to the gold patches from repository developers, revealing limitations in the benchmark's test case coverage. Most agents maintained code reliability and security, avoiding new bugs or vulnerabilities; while some agents increased code complexity, many reduced code duplication and minimized code smells. Finally, agents performed better on simpler codebases, suggesting that breaking complex tasks into smaller sub-tasks could improve effectiveness. This study provides the first comprehensive evaluation of agent-generated patches on real-world GitHub issues, offering insights to advance AI-driven software development.

==> sections/discussion_of_future_work.tex <==
\section{Discussion of Future Work}

In our exploratory study, we have found that AI agents exhibit different modification behaviors, such as changing different files and functions compared to repository developers and maintainers. We also evaluated non-functional metrics of the agents' generated code, focusing on reliability, security, and maintainability perspectives.

In our future work, we will continue to analyze \textbf{conformance}, \textbf{error handling}, and \textbf{recovery strategies} in these software development agents. As AI agents become more popular and are considered for deployment to automate many software development tasks, it is crucial to ensure not only their programming ability but also their stability and reliability---especially before deploying them in critical systems like air traffic control or defense systems. Therefore, we will analyze several thousand trajectory files from dozens of top-ranked agents on the SWE-bench leaderboard.

Our planned steps are as follows:

\begin{enumerate}
    \item \textbf{Workflow Extraction}: We will extract agent developer-designed key actions, decisions, and steps from each agent's trajectory to discover predefined agentic workflows.

    \item \textbf{Conformance Checking}: By comparing agents' actual processes against the originally planned agentic workflows, we aim to identify deviations that could be dangerous or lead to loss of human control. To perform this conformance checking, we will use the RAG technique, which allows for effective assessment of adherence to expected workflows. Ensuring agents adhere to expected workflows is essential for safety and predictability.

    \item \textbf{Error Identification}: We will use NLP techniques to detect mentions of errors or failures in the trajectories. \emph{Understanding where and why agents encounter errors will help us identify vulnerabilities and areas that require improvement, which is vital for enhancing their robustness.}

    \item \textbf{Strategy Extraction}: We will analyze subsequent actions to see how agents respond to errors. \emph{By examining their recovery strategies, we can assess their resilience and ability to handle unexpected situations, which is critical for reliable deployment in high-stakes environments.}

    \item \textbf{Comparative Analysis}: We will compare strategies across agents to determine which are most effective, providing insights into best practices for error handling and recovery.
\end{enumerate}

Overall, our potential contribution is to provide insights into the \textbf{conformance} and \textbf{stability} of AI agents, enhancing AI resilience and reliability in software development tasks.


==> sections/experiment_setup.tex <==
\section{Experiment Setup}
This section describes the specific experimental settings implemented to provide answers to each research question.


\subsection{Base Model}
\label{sec:model_choice}

